Lifting C Semantics for Dataflow Optimization

C is the lingua franca of programming and almost any device can be programmed using C. However, programming mod-ern heterogeneous architectures such as multi-core CPUs and GPUs requires explicitly expressing parallelism as well as device-specific properties such as memory hierarchies. The resulting code is often hard to understand, debug, and modify for different architectures. We propose to lift C programs to a parametric dataflow representation that lends itself to static data-centric analysis and enables automatic high-performance code generation. We separate writing code from optimizing for different hardware: simple, portable C source code is used to generate efficient specialized versions with a click of a button. Our approach can identify parallelism when no other compiler can, and outperforms a bespoke parallelized version of a scientific proxy application by up to 21%.

==> img/figpb.tex <==
\begin{figure*}
\begin{tikzpicture}
    \begin{axis}[
    title={2mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        ylabel = {\small Time (seconds) },
         y label style={at={(0.4,0.5)}},
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
   \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.2,0.6,1,1.4,1.8,2.2},
%xticklabel style={align=center},
xticklabels={{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $},{\tiny $ $}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
\begin{tikzpicture}
    \begin{axis}[
    title={2mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        ylabel = {\small Time (seconds) },
         y label style={at={(0.4,0.5)}},
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
   \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}
     \begin{tikzpicture}
    \begin{axis}[
    title={3mm},
        width  = 0.17*\textwidth,
        height = 3cm,
        %major x tick style = transparent,
        ybar=1pt,
        bar width=6pt,
        ymajorgrids = true,
        xtick={0.25,0.6,1,1.4,1.8,2.15},
%xticklabel style={align=center},
xticklabels={{\tiny $SDFG$},{\tiny $Parallel SDFG$},{\tiny $GCC$},{\tiny $ICC$},{\tiny $Polly$},{\tiny $Pluto$}},
        %xtick = data,
 xticklabel style={rotate=90},
 ticklabel style = {font=\tiny},
    %    scaled y ticks = false,
        ymin=0,
        xmin=0,
        xmax=2.4
    ]

        \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.9)};
      \addplot[style={red,fill=red,mark=none}]
              coordinates {(1.2, 0.2)};
 \addplot[style={green,fill=green,mark=none}]
              coordinates {(1.2, 1.5)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.4)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.3)};
              
 \addplot[style={blue,fill=blue,mark=none}]
              coordinates {(1.2, 1.1)};

    \end{axis}
    \end{tikzpicture}    
\caption{Polybench runtime}
\label{fig:evalpb}
\end{figure*}

==> table.tex <==

\begin{table}
\footnotesize
\begin{tabular}{p{0.50in} p{0.4in} p{0.6in} p{0.5in} p{0.6in}}
\toprule
 
  &	        & \multicolumn{2}{c}{\bf Depth}      &\bf Average  \\
\bf  \bf Kernel       &	\bf Work            & \bf hand-tuned                 &\bf      auto     &\bf Parallelism  \\
\midrule
%Declarations &\\
%\hline
2mm  &  	 $2N^3$ &	 $2\log(N)$ &	 $5\log(N)$ &	 $2N^3/(5\log(N))$ &  \\ 
3mm  &  	 $3N^3$ &	 $2\log(N)$ &	 $4\log(N)$ &	 $3N^3/(4\log(N))$ &  \\ 
adi	 & $6N^2t$ &	 $4N \cdot t$ &	 $4N \cdot t$ &	 $3N/2$ &   \\ 
atax  &  	 $2N^2$ &	 $N\log(N)$ &	 $2\log(N)$ &	 $N^2/\log(N)$ &  \\ 
bicg  &  	 $2N^2$ &	 $2\log(N)$ &	 $\log(N)$ &	 $2N^2/\log(N)$ &  \\ 
cholesky  &  	 $N^3/6$ &	 $N^2\log(N)/2$ &	 $N^3/6$ &	 $1$ &  \\ 
{correlation}  &  	 $N^3/2$ &	 $3\log(N)$ &	 $N^2\log(N)$ &	 $N/(2\log(N))$ &  \\ 
covariance  &  	 $N^3/2$ &	 $2\log(N)$ &	 $N^2\log(N)$ &	 $N/(2\log(N))$ &  \\ 
deriche  &  	 $20H\cdot W$ &	 $4H\cdot W$ &	 $14H\cdot W$ &	 $10/7$ &  \\ 
doitgen  &  	 $N^4$ &	 $\log(N)$ &	 $2N\log(N)$ &	 $N^3/(2\log(N))$ &  \\ 
durbin  &  	 $3N^2/2$ &	 $N\log(N)$ &	 $N\log(N)$ &	 $3N/(2\log(N))$ &  \\ 
fdtd2d  &  	 $3N^2T$ &	 $3T$ &	 $2T$ &	 $3N^2/2$ &  \\ 
floyd-war.  &  	 $2N^3$ &	 $\log(N)$ &	 $N^3$ &	 $2$ &  \\ 
gemm  &  	 $N^3$ &	 $\log(N)$ &	 $2\log(N)$ &	 $N^3/(2\log(N))$ &  \\ 
gemver  &  	 $3N^2$ &	 $2\log(N)$ &	 $2\log(N)$ &	 $3N^2/(2\log(N))$ &  \\ 
gesummv  &  	 $2N^2$ &	 $2\log(N)$ &	 $N$ &	 $2N$ &  \\ 
gramschmidt  &  	 $N^3$ &	 $2N\log(N)$ &	 $2N\log(N)$ &	 $N^2/(2\log(N))$ &  \\ 
heat3d  &  	 $2N^3t$ &	 $2t$ &	 $2t$ &	 $N^3$ &  \\ 
jacobi1d  &  	 $2N \cdot t$ &	 $2t$ &	 $2t$ &	 $N$ &  \\ 
jacobi2d  &  	 $2N^2t$ &	 $2t$ &	 $2t$ &	 $N^2$ &  \\ 
lu  &  	 $N^3/3$ &	 $N^2\log(N)/2$ &	 $N^3/3$ &	 $1$ &  \\ 
ludcmp  &  	 $N^3/3$ &	 $N^2\log(N)/2$ &	 $N^2\log(N)$ &	 $N/(3\log(N))$ &  \\ 
mvt  &  	 $2N^2$ &	 $2\log(N)$ &	 $\log(N)$ &	 $2N^2/\log(N)$ &  \\ 
nussinov  &  	 $N^3/3$ &	 $2N^3$ &	 $N^3$ &	 $1/3$ &  \\ 
seidel2d  &  	 $N^2t$ &	 $N^2t$ &	 $N^2t$ &	 $1$ &  \\ 
symm  &  	 $N^3$ &	 $\log(N)$ &	 $3N$ &	 $N^2/3$ &  \\ 
syr2k  &  	 $N^3/2$ &	 $\log(N)$ &	 $2\log(N)$ &	 $N^3/(4\log(N))$ &  \\ 
syrk  &  	 $N^3/2$ &	 $\log(N)$ &	 $2\log(N)$ &	 $N^3/(4\log(N))$ &  \\ 
trisolv  &  	 $N^2$ &	 $N\log(N)$ &	 $N\log(N)$ &	 $N/\log(N)$ &  \\ 
trmm  &  	 $N^3/2$ &	 $\log(N)$ &	 $N^2\log(N)$ &	 $N/(2\log(N))$ &  \\ 


%\multicolumn{4}{l}{\alex{and all the others once they are correct}}\\\addlinespace
\bottomrule
\end{tabular}
\caption{Lead order term work depth analysis of Polybench .}
\label{table:wd}
\end{table}

